We Do Not Understand What It Says -- Studying Student Perceptions of Software Modelling

Background: Despite the potential benefits of software modelling, developers have shown a considerable reluctance towards its application. There is substantial existing research studying industrial use and technical challenges of modelling. However, there is a lack of detailed empirical work investigating how students perceive modelling. Aim: We investigate the perceptions of students towards modelling in a university environment. Method: We conducted a multiple case study with 5 cases (5 courses from 3 universities) and two units of analysis (student and instructor). We collected data through 21 semi-structured interviews, which we analysed using in-vivo coding and thematic analysis. Results: Students see some benefits of modelling, e.g., using models for planning and communicating within the group. However, several factors negatively influence their understanding of modelling, e.g., assignments with unclear expectations, irregular and insufficient feedback on their models, and lack of experience with the problem domains. Conclusions: Our findings help in understanding better why students struggle with software modelling, and might be reluctant to adopt it later on. This could help to improve education and training in software modelling, both at university and in industry. Specifically, we recommend that educators try to provide feedback beyond syntactical issues, and to consider using problem domains that students are knowledgeable about.

==> Extra stuff/Analysis.tex <==
\subsection{coding: 26th Jan- BTH}
\newcommand{\interviewquote}[2]{\begin{quote}
\footnotesize{\emph{``#1'' }} --- \footnotesize{#2}
\end{quote} }

\interviewquote{"So the reason it's like you can't be mustering everything and more into implementation rather than modeling things"}{BTH\_PASE\_S2}- preference.
% students with industry experience provides good reasoning towards their challenges for modelling.%
\interviewquote{"The reason is like, I have much experience to allow for the implementation"}{BTH\_PASE\_S2}


%planning the development, talking about assignments. %
\interviewquote{When we do with planning, it's very easy}{BTH\_PASE\_S3} 
\interviewquote{But in this kind of planning, in this kind of thing, you have divided into parts into chunks. So when you are writing your partner chunks, you can take out only one or two things from where you get the mistakes. So it's very easy.}{BTH\_PASE\_S3}
\interviewquote{We are stuck in agile.}{BTH\_PASE\_S3}
\interviewquote{But I think that we should teach our students about devops, because devops is one of the best thing in the market}{BTH\_PASE\_S3}
%learning experience%
\interviewquote{I have done two types of learning. One is in the form of group and one is individual individual. There are benefits, different benefits and individual learning, and there are different benefits and problems in individual learning. You only talk about one mind. You only talk from one mind and you have one mindset. You don't think about other material. Other things. OK, but in group, you get your money like you are supposed to think like what you are thinking should be different from other. Because if one is saying you that from my side, this is the thing and that this is not OK in group. You have to do something different. Everyone should do different things. From there, we get a more robust kind of information, what kind of information to get to implement in our system.}{BTH\_PASE\_S3} about learning.
%Group work- here its interpreted as positive, not a challenge%
%previously we have seen group issues as a challenge. Interestingly, that challenges came from students who have industry experience/experience in coding. Here, BTH_PASE_S3 is a beginner and new in modelling%
\interviewquote{Well, our minds think different. At the end of the day, we have to do the same.}{BTH\_PASE\_S3} 
\interviewquote{If one is one of our group members thinking wrong, then when he will come back to us with that information, we can teach him. No, it's not in that form. It's like in that form. So it's a very good thing.}{BTH\_PASE\_S3}
%Also a beginner in modelling but have industry experience in some other field%
\interviewquote{when you're doing so assignments and everything with a group because everyone has a different point of view and there's going to be very messy}{GU\_S_S2}
%challenges: covid issues%
\interviewquote{There was a problem that is well in online classes and in online meetings. No one can give so much didn't mean discussion about things.}{BTH\_PASE\_S3}

\interviewquote{in start, it was difficult, but the time to time when our teacher was very cooperative}{BTH\_PASE\_S3}
%tooling: not very specific towards modelling tool: student thinks its a good thing%
\interviewquote{There was not like proper software like Android, like we use really like anything that kind of. It was just like simple. Very simple.}{BTH\_PASE\_S3}
\interviewquote{We are free to use any tool. And that's a good thing because course in bachelors we are forced to the only thing we are forced to do, only C++, then C# every teacher has because every teacher has his own command on that}{BTH\_PASE\_S3}
\interviewquote{And but it was quite good working with the new things like it also have the opportunity to you can choose any platform to develop the thing from your leg room}{BTH\_SAQ\_S2}

%when modelling is useful%
\interviewquote{ And I think we just what do you have a calculator we start coding at the end of the day, if you don't know what we did? We don't know because only we know coding. But if you want to make calculator and if you will define it, function properly in one picture and then you can implement one one feature. Exactly. And then you can test and then you can report. It's a proper project.}{BTH\_PASE\_S3}
\interviewquote{As I told you, the advantage is that sort of become easy to build for you and disadvantage. It consumed time.}{BTH\_PASE\_S3}
%student suggestion%
\interviewquote{We should know about the basics of tech. This tool is in market. We should know the basics there. But is this how it is implemented? What things are important for what it is and where there is too much hype of Florida that we should know about these things also besides theory and more.}{BTH\_PASE\_S3}

%impression about modelling%
\interviewquote{Honestly, I should say. And I would say I never saw the draw use case or diagrams. They just note that talked about the system and go for implementation even are unlikely to just convey some information from his understanding or his maybe interest to develop. So they start to implement the software development, no the use case, even context.}{BTH\_SAQ\_S1}
\interviewquote{Or you can actually in real world, such things happen maybe during a practice practice or not, but I didn't. So just in academia.}{BTH\_SAQ\_S1}7
\interviewquote{ You know, if you may say that it's if I need something I have to go in the in the code level are to develop a system. So in that case, I think your UML is not giving any benefit to us.}{BTh\_SAQ\_S2}

%learning challenges%
\interviewquote{Actually, it's this and it's about, you know, the examples are about the device, not what software}{BTH\_SAQ\_S1}
\interviewquote{ we have some problem because it's not easy to discuss}{BTH\_SAQ\_S1} B39
%the student is asking about the process.%
\interviewquote{No, actually, I'm not satisfied because they just they don't have some raw material and expect us to our input, so have been so precise and in detail, but by just by learning no about and following some example, for me, it's not feasible}{BTH\_SAQ\_S1}
%Lacking modelling efforts in company%
\interviewquote{but my problem is maybe the companies should define a role for some expert people to create it and, you know, use case or diagrams quickly and in a good way}{BTH\_SAQ\_S1}

\subsection{Patterns}
\begin{itemize}
    \item The issues we got (section 10.1) in our last analysis, are those still applicable in this analysis?
    \item All 6 students from BTH are Asian. Any interesting pattern among those data? 
    \item Connection between challenges and student groups? 
    \item Is communication most popular issue among beginners?
    \item Two types of challenges: common challenges (such as, modelling is time consuming, going back to diagram while coding etc) and specific challenges (such as,challenges regarding the assignments or tasks, personal difficulties etc). Example for specific challenges: BTH\_SAQ\_S2 Cell-B37
    \item when modelling is not useful and when modelling is not done: two different things. G1 answers the second question. 
\end{itemize}

\section{Themes/ Description}
\begin{itemize}
    \item Challenges/``Bad": What is challenging for a student in terms of modelling? Can be grouped into two sections: challenges regarding learning modelling and challenges regarding appluing modelling 
    \item Purpose/``Good": 
    \item Course Setup/``What?":
    \item Preferences/ ``Why?":
\end{itemize}

\section{Codes\_students}
\shalini{The analysis right now is based on data from first 4 students of GHOH (RU\_G\_S1, RU\_G\_S2, RU\_G\_S3 and RU\_G\_S4) and one student from SRAD (RU\_S\_S1).}
            \begin{enumerate}
                \item \textbf{Same Page:SP} Modelling helps everyone to be on the same page. Most popular opinions from the students were regarding this purpose, communication. According to students they used modelling to communicate between themselves.  
                \interviewquote{Modelling is very important for communication and documentation.}{RU\_G\_S3}
                %
                
                \interviewquote{Well, advantage, as I say, is the best way to communicate, it's the best way to comment, and best way to-- Yes, mainly to comment, and think, and advice}{RU\_G\_S3}
                %
                
                \interviewquote{We modelled sometimes state diagrams, but not professionally. It's more to communicate between me and my colleague}{RU\_G\_S3}
                %
                
                \interviewquote{If the design was more close to the end product, it would be more easy to communicate with the group}{RU\_G\_S3}
                %
                
                \interviewquote{I think it's important for documentation, as well as getting everyone on the same page}{RU\_S\_S1}
                %
                
                \interviewquote{I was having a target to have the highest best product in our crew work, but not everybody want this. This difference of target makes miscommunication also. The class modeling of course, class modeling. Modeling is very, very important to make everybody on the same page at least.}{RU\_G\_S3}
                %
                
                \interviewquote{It's useful for documenting and getting everyone on the same page, I think. I've learned a lot and because I've taken a lot of design classes, basically three people can be talking about the same thing and they can write everything down, what they're talking about and they all think they have the same idea, but they actually have a very different idea, everyone but as soon as you draw it up on a whiteboard or create a diagram of it, you're definitely sure that everyone is on the same page. I think it's really useful for getting everyone on the same page, probably.}{RU\_S\_S1}
                %
                
                \interviewquote{Big companies also, when we have a lot of department, or even one department, but many workers, usually in the same project, it's very important to have standard between the worker, so not two guys think for same problems different way. They have all to follow the same design, which is the model. It helps everybody to be on the same page}{RU\_G\_S3}
                %
                \item \textbf{Planning Ahead:PA} To understand the given problem through modelling, later they implemented the model (although that was required for the course). 
                \interviewquote{Class diagrams what we had was like a bigger version of the app and we saw the connection between the classes, between the models, and the structures in the app. We could easily go back and front and how to connect the dots instead of just writing the code and then just looking the connections in the codes. I could actually just look at one picture and I knew what's happening in there. It was just easier for me to understand it.}{RU\_G\_S4}
                %
                
                \interviewquote{Advantages? I think simply one is just it's going to be easier for you later on when you start to program the app, I'm telling you, it's way simpler for you. You just don't even have to think it, it's just like you have to follow the scheme of the diagrams and all that, and just connect it in the app, and it goes like this}{RU\_G\_S4}
                %
                
                \interviewquote{But the thing I liked this is when you feel like you have a plan and you know what are you gonna do}{RU\_G\_S2}
                %
                
                \interviewquote{...but then I guess, the design of the system as a way to communicate and document the design, and thinking in advance how to solve this problem. How is this useful? It's very useful, of course, because it saves a lot of time, and of course, money for big company, because you can find the problem before you design-- Before you implement. You can fix the problem in a design, which is much easier and faster to fix before you implement it}{RU\_G\_S3}
                %
                
                \interviewquote{For every phone app or for any-- even a website or anything that you're going to program, making a good model of the app before starting doing it is very important||Usually, in most cases, it's always very important to have a good background in the model and the diagrams before you're going to program anything}{RU\_G\_S3}
                %
                \item \textbf{Handling complexity:HC} Another approach from students. It's their way of understanding the problem or the complexity of the problem. One of the purpose of modelling for students. 
                \interviewquote{ I think when you have an idea for the app, you have to think about the structure of the app and how it's going to look like. It's just like model of the app, it's just like way before writing the app. It's like all the design process. I think this is what you mean by modeling the app.}{RU\_G\_S4}
                %
                
                \interviewquote{It depends on how much of a detail you want to go into. If you're creating a small REST API, it can be good to create just a small high-level class diagram that basically says, "Here's the class that handles the API requests. Here is the database connection layer, here is the logic part or something." Basically, just to see how everything connects together...}{RU\_S\_S1}
                %
                
                \interviewquote{The simplicity of connecting everything together, you can just create a box, name it for this is a class, name it, and then you can just drag this, connect to this one}{RU\_S\_S1}
                %
                
                \interviewquote{So then we understood how like after being able to do the class diagrams which was extremely difficult for us to do or understand or wrap our heads around but once we did the diagram we like understood}{RU\_G\_S2}
                %
                
                \interviewquote{What we did was we created a diagram that contained all the classes, but no detail about the classes. Basically, just how the class interacted and in what container they were kept, and then we went into the details of each and every class. That's basically how I work with UML, I just start as high as I can and just split it down}{RU\_S\_S1}
                %
                
                \interviewquote{Because we had this physical model representation of the program}{RU\_G\_S1}
                %
                
                \interviewquote{If you are making a program that has more than 200 lines of code then you probably gonna have to model it. }{RU\_G\_S1}
                %
                
                \interviewquote{In each sprint, we basically refactored the whole code that we had written. In the first sprint, we created the rest API with a lot of duplication of code, and if we had made a diagram of that, we would probably have to teach it and create a new one on the second sprint. I think that getting the idea as a whole, in the beginning, is better for me, I think}{RU\_S\_S1}
                %
                
                \interviewquote{But if you making something that you create something, you read out of it and you, you look at it and stuff, then you gonna have to use programs to really just  trace back n forth through the, through the model to better understand what you doing}{RU\_G\_S1}
                %
                \item \textbf{Usefulness:US}
                \grischa{Isn't this a category that contains SP, PA, and HC?} Not so much data here; although changing the model often seems a problem for students, they still think it's better to make changes at the modelling level than later at programming. The usefulness of modelling is in communication, documentation, complexity handling etc. 
                \interviewquote{Modeling is very important and very effective, and even if it's not big company, if it's a one-person application, it's very important, because in the future you forgot why you make something.}{RU\_G\_S3}
                %
                
                \interviewquote{Yes, modeling is important at all levels, I think. It's taking some time, it's more faster if you implement it right away, but it's very critical, especially in the maintenance time, when you have to maintain the software. Usually, it's another people who will maintain software, so they need to read what you make if they need to understand. It's a very basic step for communication documentation for making everything, life easier for everybody}{RU\_G\_S3}
                %
                
                \interviewquote{The main advantages, I think, is when you are trying to get to a solution, the modeling can really help you basically get an overview of your whole solution and also just for documentation. It basically helps you solve a problem outside of code because changing code is a lot harder than tainting a small table in a model. You're a lot faster at making changes when you're doing the UML diagrams or just other diagrams or models.}{RU\_S\_S1}
                %
                \item \textbf{Modelling something because of inexperience:MInEx} This group of statements explains that students are actually confused about modelling. One of the main challenges students face is to change the model multiple times. They even changed their diagrams after programming. "...lot of people thought it was (class diagram) kind of pointless to begin with...in the very end they pretty much didn't follow the class diagram at all."
                \interviewquote{Of course, the main challenge was to actually do it perfectly at one go because...}{RU\_G\_S4}
                %
                
                \interviewquote{we had to, we had to basically just create a class diagram out of the code that they wrote, instead of writing a code out of the class diagram}{RU\_G\_S1}
                %
                
                \interviewquote{Probably the biggest challenge I faced, was creating a UML diagram, programming something, and needing to change it later. In the first course on the first semester, we changed the class diagram, I think five times because we designed something, it didn't work, so we needed to change it and then we had to design it again basically.}{RU\_S\_S1}
                %
                
                \interviewquote{Yes. The first week was creating class diagrams and a few sequence and I think we also had to create an activity diagram. Then basically we had to design the system from that and that was why we had to change it four times because when we started designing the system, our original design wasn't really good or didn't work really well, so we just had to create it again.}{RU\_S\_S1}
                %
                
                \interviewquote{I think basically the problem we had in the three records was that we had never done anything like it before, we had never built the whole system. It was more like we were learning new stuff and changing the model afterwards. I think that's the main reason it was a problem for us but in the sprints, because we were only creating the diagrams in the full sprint, we didn't need to change anything, it was more like just the documentation, but if we had to model each sprint, it would have been really a big problem because we changed everything.}{RU\_S\_S1}
                %
                
                \interviewquote{...but if we had to model each sprint, it would have been really a big problem because we changed everything.}{RU\_S\_S1}
                %
                
                \interviewquote{I have to point out that we were not the best people at using the knowledge to design it because later on, we had to fix it at least 10 times. After writing the app, we had to go back to our diagrams and redo them how our final vision was. I think my experience is not very high experience. I wouldn't define it as that. I think it's very important to prepare a good structure for the app or for anything because that's really helped the people later on with the programming.}{RU\_G\_S4}
                %
                
                \interviewquote{But we had to do this, this class diagram and everyone just, well a lot of people thought it was kind of pointless to begin with and i remember many groups saying that in the very end they pretty much didn't follow the class diagram at all}{RU\_G\_S1}
                %
                \shalini{Changing the model was a big problem for students. They did not understand the purpose/concept in the beginning}
                \grischa{Yes. This code should maybe not be DKD, but more "rework due to inexperience" or "modelling something because of inexperience"}
                \item \textbf{Timing:T} Modelling is time consuming. 
                \interviewquote{Disadvantage. I think time-consuming because it takes time to design it}{RU\_G\_S4}
                %
                
                \interviewquote{Yes. That's the problem, is how much time you have}{RU\_G\_S3}
                %
                \item \textbf{Challenges in general:C} "We are just drawing diagrams"-clueless about the purpose. They are questioning what is the need to learn different types of diagrams? or Modelling?
                \interviewquote{The main disadvantage is, I'm not sure. Maybe just that it takes time if you're doing a small project. Some projects don't really require maybe a modelling session if they're small enough.}{RU\_S\_S1}
                %
                
                \interviewquote{a lot of people actually disliked the UML course because they thought it was pointless. Basically, it was just, \textbf{We're just drawing diagrams.}}{RU\_S\_S1}
                %
                
                \interviewquote{No it was not, because mainly we were branch in a company for recession development. We are not a software house, we are a stock market company, and we are the branch who make software for the company. We mainly the team was only two, but I work in other company where we have more people, but we didn't follow also the modeling system, everybody makes from two or three persons had the same application.}{RU\_G\_S3}
                \shalini{lacking practices?}
                \interviewquote{What I dislike? Probably the lack of cooperation with draw.io. I know that you can cooperate like we've done where you can just save the diagram, in a draw.io folder, but then usually if one person changes it, it takes 15 to 20 seconds for the other person to see it}{RU\_S\_S1}
                \shalini{Tool issue}
                \interviewquote{I would probably actually introduce a problem that is really hard to fix without modelling and maybe either make them solve it or show them how to solve without modeling and then I would actually show them how to solve it when it's modelled first because a lot of people actually disliked the UML course because they thought it was pointless}{RU\_S\_S1}
                %
                \item \textbf{Practice/Guidance:P/G} They learn about modelling but don't get to experience modelling: lack of practical exposure, different outcomes from different teacher, short practise time.
                \interviewquote{I got enough knowledge but I didn't get enough experience|| I just got all the basic knowledge, a little bit of advance in that but mostly basic knowledge, not a lot of experience.}{RU\_G\_S4}
                %
                
                \interviewquote{The practical side, we need more. Somehow the group work, don't make sure that everybody understands. We are six, for example, but one or two would make the modeling and the rest maybe don't understand. Somehow, I don't know how to solve this problem. If the school didn't focus, and maybe the school need to be sure that every part and group had understand the sign or have part on it.}{RU\_G\_S3}
                %
                
                \interviewquote{We did it in phases, so I didn't really get much of experience on that because I was just following the sketch that we got in the lectures and the classes and just tried to gather the basic stuff, designing in my head}{RU\_G\_S3}
                %
                
                \interviewquote{I think what I would say was not enough practice on the classes and being people learn more about it when they do it in practice. When we were at school, we were mostly going over the lectures, the basic stuff, and how it's supposed to look like. I think we didn't really know how it should look like in the big picture. It was one semester, we got to know all the basics and the whole idea and how it's supposed to look like, but not how to use it in the future on the bigger picture and the scale of the app. That was the biggest challenge when they're using it}{RU\_G\_S4}
                %
                
                \interviewquote{Mainly we have little time, me and my colleagues because we are working, except two member, we were six||Technically, I think at one point if we try to give the design more time, we could finish it more easy, a more perfect, more close}{RU\_G\_S3}
                %
                
                \interviewquote{Maybe because it's the first year, this is the first introduction to the subject, so people miss a lot of points, but if it had another level, teach people more, and take their hand more to do these diagrams themselves, that would be good}{RU\_G\_S3}
                %
                
                \interviewquote{Felt like when it really came down to it, the UML part should have been a lot more. Because that we ended up using a lot}{RU\_G\_S1}
                %
                
                \interviewquote{I think this is more missing in the master's course, that every week, we would have a small assignment that we could just practice because I think mostly, I didn't get enough experience. We just had a big group project, which was three weeks to two weeks long. I think the teacher also didn't give much feedback on the assignments so I think that was missing, a feedback part from the teachers, if we were doing it correctly, if it doesn't look good, or anything like this. I think the experience is missing.}{RU\_G\_S4}
                %
                
                \interviewquote{It needs another level to teach them the other diagrams and teach them more deeply about the system. That's it. They didn't teach us all the modeling. It was good for first year, but maybe if it's another course with more modeling diagrams, and more practical, like when we make the semester project. Most of the guys don't know, even after they finish the course how to design the diagram correct. Not most, but some guys.}{RU\_G\_S3}
                %
                
                \interviewquote{To design that, on academic level, I'll probably have at least two or three lecture slots per week, where we go over book stuff so we go over the book and what's the knowledge we need to have sufficient knowledge about modeling. I think once a week for three, four hours, I would do a lab session, that we go over problems, and there would be a small assignment every week that we practice ourselves on the lab session. Then every two weeks, we will have a bigger group assignment, like we had on the master's course, that we would just follow one big app skit, and we'll find some idea to design some app like we did at masters.}{RU\_G\_S4}
                %
                \item \textbf{Group Issues:GI} The assignments were in group, different students have different opinions. Less professionalism. 
                \interviewquote{For example, you can give an effort in one design, but your colleague will never look at it. That could be easy going. That could happen in the school. You can lose communication not only because of design, no, because your colleague not willing to study design or not willing to collaborate, one point for any reason}{RU\_G\_S3}
                %
                
                \interviewquote{We don't usually give it time, because we finish the design not complete, so the picture, the end picture is not clear with everybody, and I want you to know something also. We are not in a high professional environment. We are a student in a class. If we are in a company, this would be different level of talk, and the level, the communication will be very high, professional.}{RU\_G\_S3}
                %
                
                \interviewquote{…but I think it would have been a lot better if we had all just sat down and done a class diagram and a sequence diagram, I think}{RU\_S\_S1}
                %
                
                \interviewquote{I have a small problem, because I have a little bit more experience than them, so I feel like I'm pushing my ideas}{RU\_G\_S3}
                %
                
                \interviewquote{Yes, this was so challenging how I can manage to make everybody happy, I'll say to somebody, "Let's not take this idea, and take this idea." This is a very, very difficult thing. I don't know how we resolve it in the next project}{RU\_G\_S3}
                %
                \item \textbf{Course issues:CI} Due to course structure, less time to learn.
                \interviewquote{I think it's more important for the people to know in what cases you can use the diagrams and all kinds of modeling stuff}{Ru\_G\_s4}
                %
                
                \interviewquote{assignment driven course}{RU\_G\_s1}
                %
                
                \interviewquote{I think it's not good idea to have two teacher, to teach one course||I find something which is not nice, actually, that both had to teach us use-cases, but they have a little bit different notation between both of them.}{RU\_G\_S3}
                %
                
                \interviewquote{I don't know how. This is a lot of work, but some people don't get involved much because it's group work.}{RU\_G\_S3}
                %
                
                \interviewquote{There was one weird thing because software engineering was changing when I started. The first course that I took, a three-week course because I hadn't learned UML before, so basically we had to learn UML in one week or less}{RU\_S\_S1}
                %
                
                \interviewquote{we got to know all the basics and the whole idea and how it's supposed to look like, but not how to use it in the future on the bigger picture and the scale of the app}{RU\_G\_S4}
                %
                \item \textbf{Model Purpose:MP} "Design first, then implement", "school forces us to model..." The purpose of modelling to students. 
                \interviewquote{school force us to model, because they want us to think this way, model and design then implement. To say the truth, if I have limited time, and I have a application, which is my own application, I would finish it mainly by sketching, and not spending time to design something on the tool or anything}{RU\_G\_S3}
                %
                
                \interviewquote{...and the diagrams had to fit the code}{RU\_G\_S4}
                %
                
                \interviewquote{At the end, we had to go back to our drawings and we had to fix them. Since we didn't have much experience in programming and designing and modeling the app, I think the biggest challenge was in the first week that we were just flowing with our ideas how the app should look like without actually knowing how the end picture of the class diagrams should look like, and what will we absolutely need when we thought about it, when we started the program was like, "Oh, we're missing this part and this part." We would be, "This is very useful that we didn't thought about in the beginning."}{RU\_G\_S4}
                %
                
                \interviewquote{but we didn't create any diagrams until the full sprint, which we thought was weird, but still, then we were more just diagrams not for problem-solving, but more for documenting what we had already done}{RU\_S\_S1}
                %
                
                \interviewquote{For the three-week course, we used all of them because it was necessary. It was the requirement for the grade but what we mostly used for our own purposes was the class diagram mostly which was the most useful. We didn't really look for the other diagrams when we programmed}{RU\_G\_S4}
                %
                
                \interviewquote{Afterwards, we all thought that the first sprint should have been only about assigning the software that we were going to create. Creating diagrams, documentation, and thinking about the solution but the first sprint was basically just, "Create something."}{RU\_S\_S1}
                %
                
                \interviewquote{This is the course rule, we have to design first and submit the design, the teacher would say his opinion, and then you'd implement}{RU\_G\_S3}
                %
                \item \textbf{Preferences:P} How the students perceive modelling and how they complete the assignments through modelling (very close to style) "...we sometimes just get something based on UML but it is not completely UML"
                \interviewquote{I always have paper and pen, so even if I can't use the software, I can sketch stuff, it's casual sketching. It's nothing professional, but at least for me to communicate to think about the problem, and model it}{RU\_G\_S3}
                %
                
                \interviewquote{The level of modeling is the idea. For me, myself I think that the enough modeling is a class diagram, because either I make it in a paper, or I make a direct in a database. Then I export the diagram as a diagram. This, I think it's always important, but it depends how much you are satisfied. Depends how much time you have. The minimum level, I think for me is class diagram, to have it at least in the database}{RU\_G\_S3}
                %
                
                \interviewquote{In the beginning, I don't model something unless I have to work with somebody, or unless I have to explain someone something. If I'm working alone, which is most of the time, I'm working for my project all alone, I used to do everything in sketching in paper. Mainly also class diagram, some state diagram, but I get used to start implement right away. Even if I have to make state diagram, I can imagine it in my brain, and start implementing, then document it}{RU\_G\_S3}
                %
                
                \interviewquote{To say the truth, if I have limited time, and I have a application, which is my own application, I would finish it mainly by sketching, and not spending time to design something on the tool or anything.}{RU\_G\_S3}
                %
                
                \interviewquote{Mainly, it was casual. If I have to work with my colleague on special task, our software we share it together, so I model mainly the class diagram, and if small state diagram, I model it to explain to him how things were going. If I'm working in a Sys.Application completely alone, I usually delay the modelling and the design. Of course, I model everything in paper as database, how communication between the component as a class diagram consider}{RU\_G\_S3}
                %
                
                \interviewquote{I do it exactly as I implemented. Especially the class diagram, because the class diagram is the database for, in my point of view, and so I use this as the base for my database. Then the component diagram which is where's the data layer, and the interface layer and show all these. This just, it's also what I implement. No, I use it in a very big level. Yes.}{RU\_G\_S3}
                %
                
                \interviewquote{It doesn't follow the principles, and as soon as we understand that nearly everything is just boxes and arrows from here to here|| If we make a file wireframe, we don't need to make all the modelling, because it explain how the system will work}{RU\_G\_S3}
                %
                
                \interviewquote{I model everything for myself just on paper and pen, and use in the same moment, I start to design in the database system. I delay the modelling until I find I have to explain to someone. It's really, [laughs] I keep it for the documentation}{RU\_G\_S3}
                %
                
                \interviewquote{When I did the prototype of my app, I used the Figma app on the internet. It's really good to visualize the prototype. Then we used the Lucidchart and draw.io, I think it's diagrams.net now. This is for the diagrams. Then we just used the whiteboard to draw it if we needed to because we just gathered together and we'd just throw it on the whiteboard and then we just translated it into diagrams or Lucidchart.}{RU\_G\_S4}
                %
                
                \interviewquote{What we did was we created a diagram that contained all the classes, but no detail about the classes. Basically, just how the class interacted and in what container they were kept, and then we went into the details of each and every class. That's basically how I work with UML, I just start as high as I can and just split it down}{RU\_S\_S1}
                %
                
                \interviewquote{I think the strength of UML is basically that not everyone follows the exact syntax. Most people like me, they will basically just take what we like about UML and we use that and sometimes just change it for my own project. I know a lot of other people do it. When we are sometimes designing software and we don't necessarily have to create diagrams, we sometimes just get something based on UML but is not completely UML.}{RU\_S\_S1}
                %
                
                \interviewquote{What we usually start doing is defining everything on a real high level. Start defining just the names of the classes or everything. That's basically getting the whole picture together and then we go into more detail.}{RU\_S\_S1}
                %
                
                \interviewquote{I like modeling a lot. It helps me basically get my idea out there a lot better. Basically, when I'm starting a project, I like modeling the higher level and just going deeper and deeper and deeper.}{RU\_S\_S1}
                %
                
                \interviewquote{Most of us actually learnt to UML really well, but sometimes you just don't have to use everything about it and some parts of it are hard to remember. Sometimes we just skip the arrows and just collect things together. I'd say, "Just use this and leave the detail for when you're actually programming something." Leave the detail out of the diagram}{RU\_S\_S1}
                %
                
                \interviewquote{We were taught like that. We just got a description and we had to find everything that was going to be a class and from the description, we had to find out if they had one too many or if there were instances or something.}{RU\_S\_S1}
                %
                
                \interviewquote{I've basically only used one. That's draw.io That's  because I've used that for database design, UML design, and because I'm used to it, I just always use it.}{RU\_S\_S1}
                %
                
                \interviewquote{I actually like drawing the diagram, so I usually use a tool called draw.io and I just think it's fun. Throwing everything and getting everything to fit nicely and perfectly together and basically just getting a whole picture of the system that I can have as a sideline of when I'm programming something on a really low level, I always know what the higher-level function is doing in the system as a whole.}{RU\_S\_S1}
                %
                
                \interviewquote{Yeah, yeah we used that because it was um..prettier, than this is the whole perfectionism thing with um, it was prettier than coding}{RU\_G\_S2}
                %
                
                \interviewquote{I think actually giving people the freedom to do what they want with the tools is really nice, because some people actually liked drawing it on an iPad or something}{RU\_S\_S1}
                \item \textbf{Solve by Modelling: SM} It is one of the approaches taken by students, trying to solve the given problem by modelling. It is related to MP, as students learn to design first.  Do they understand the problem through modelling first? or just start with modelling cause it was the requirement for a course?
                \interviewquote{Basically, what we started was how to create first, how to make a prototype of the app or anything that we do. Then design, it, conduct the interviews of the people and see how actually the users' feedback is on the prototype. Then just fix the prototype and design the diagrams based on the prototype and how to do-- Like before we start to program the app, how the app is going to look like and how the diagram looks like}{RU\_G\_S4}
                %
                
                \interviewquote{First in a course, we have only problems, and we have to design it according to what she asking us to do, class diagram, state diagram. In the end project was a full project, it had all the phases from design to implement, and decremental choice. First of all, of course, we started by solving the problem by modeling it}{RU\_G\_S3}
            \end{enumerate}
%
Do the students understand a problem by modelling or start with modelling cause the course demands "design first, then implement". If we see PA (planning ahead), it seems students use modelling to understand the problem, but they complain the course demands design first.

\subsection{Codes\_instructors}
\label{sec:codes_instructors}

Regarding instructors we studied the data, their corresponding in-vivo coding and decide 6 categories:
    \begin{enumerate}
        \item Student's challenges (SC): This category describes student's challenges in modelling courses observed by the respective instructors. It contains complains from students, feedbacks regarding assignments and general doubts asked by students during projects/lectures.   
        \interviewquote{"...students complain about in this course is that everything is so undefined"}{I1}
        \item Instructor's challenges (IC): This category describes challenges faced by instructors while teaching the course. 
        \interviewquote{"I think its hard to motivate some of the students"; "...get them to understand that this an important part of software development."}{I1}
        %
        
        \interviewquote{"to fit everything into, into the project"}{I3}
        \item Modelling performed in the course(MPC): This category describes how the modelling part has been executed in the course, which includes assignment structures, project execution, the way modelling has been taught.  
        \interviewquote{"just make people literate basically in modeling so that they can observe diagrams and understand them without necessarily being able to describe complex systems using the same models"; "just make people literate basically in modeling so that they can observe diagrams and understand them without necessarily being able to describe complex systems using the same models"}{I2 (SRAD)}
        \item Modelling strategies from instructors (MSI): This category contains strategies instructors have taken or thinking of taking to improve the course. 
        \interviewquote{"That's one of the first ways to learn is that if you can explain it, you understand it"}{I2(SRAD)}
        \item Instructor's perception (about the course/assignments/students etc) (IP): This category describes an instructor's overall course perspective. How students perceive modelling, the outcome of the project etc, are covered in the category. 
        \interviewquote{"It's also my experience that the students that are studying software engineering they tend to do a bit better."}{I2(SRAD)}
        %
        
        \interviewquote{"my feeling is my gut feeling is this are two groups. Either they know it and it is easy or they have no clue and then you get weird stuff."}{I3}
    \end{enumerate}
%
\subsection{Additional statements that fall into more than one code category or new category}
\interviewquote{...I basically did class diagrams, but not with the whole UML dialect that basically used what I wanted to use in my own way. It was basically just so that I could split everything up and see what I was going to make and decide, "Okay, I can start with this thing and this is a separate from everything else, basically just more to..." I think it's useful also basically to just plan what you're going to build.}{RU\_S\_S1}
\shalini{This statements sounds like ``planning ahead" and/or ``handling complexity"}
%

\interviewquote{It's also how much enough modeling, you can say, "It's enough for me, it's enough modeling is to make the class diagram. The rest is just in my brain." Some people, "No, it's enough for us to make state diagram, class diagram, sequence diagram."}{RU\_G\_S3}
\shalini{How much modelling you need? Maybe falls under preference?}
%

\interviewquote{I think that introducing the reason why we have to model something is really smart to do in the beginning}{RU\_S\_S1}

\subsection{Student need/expectation to see examples}
Students express the need to get examples that they can copy or imitate. They are confused by the way it's taught, i.e., they have to model first, and are then corrected.
Does this mean they really need the examples to learn better, or is this just an expectation?
19:31 "I always need to google that"
21:10 "not taught right from day 1"
21:40 "I will want a blueprint"

\subsection{Student Groups}
%
We identify 3 groups among the student interviewees:
\shalini{Try to create an overview where the student groups are somehow connected to the modelling challenges}
\begin{itemize}
    \item \textbf{G1: Experienced in coding (e.g. BTH\_PASE\_S2)}
    Members of this group are experienced in coding, majority of them have worked in industry before.  \newline
    \textbf{Properties}: provide strong statements, either dislike or have less experience in modelling  \newline
    \textbf{Examples}: \interviewquote{The reason is like, I have much experience to allow for the implementation.}{BTH\_PASE\_S2} 
    \interviewquote{So like, that's not, I'm not that much interested in it, and I don't have enough experience for the documentation...}{BTH\_PASE\_S2}
    
    
    \item \textbf{G2: Beginners/less to none working experience}
    Members of this group have little to no prior knowledge about software modelling. The majority of them are taking the course for the first time. Usually, students in this group show positive yet weak opinions about modelling. By weak, we mean their opinion is mostly about agreeing with the instructor. \newline
    \textbf{Properties}: Most confused, agree with teachers, asks lots of questions, positive towards modelling but often can't provide a strong supporting statements. \newline
    \textbf{Example}: 
    
    \item \textbf{G3: Versatile} 
    This group has a diverse population with properties similar to both G1 and G2. Some members have previous working experience, and some are a novice. However, the one characteristic that makes this group of people distinct is adapting to learning (change?). The students from this group show strong positive attitudes towards modelling, and they have the logical reasoning to support their statements. While asked they provide strong statements for modelling (in some case people with industry background provide examples in favor of modelling).\newline
    \textbf{Properties}: Clear mind, less confusion, often provide good examples to show why that individual needs to learn modelling. \newline
    \textbf{Examples}: 
    
\end{itemize}
\shalini{Students coming from different work experience but now learning modelling (BTH\_PASE\_S1): confused? similar to G2? \newline
Learning challenges: learning in a group vs individual. Is this a common problem for G2?}
\shalini{Support each group with interview statements}
%


\interviewquote{You have a very short time .. you don’t want to waste your time..I prefer to just answer as the person}{BTH\_SAQ\_S3}
        %
        \interviewquote{Disadvantage. I think time-consuming because it takes time to design it}{RU\_G\_S4}
        %
        \interviewquote{modelling takes a lot of time from us}{GU\_S\_S2}
        
        \item \textbf{Remote issues:} 
        \interviewquote{challenges, ok in start we face some kind of difficulties, like everyone was from different places and you know, there is no nothing on campus and everything is happening in line }{BTH\_PASE\_S3}
        
        \item \textbf{Group issues:} Students mentioned difficulties about working in a group. Although it might be a general challenge and not related to modelling but it would be interesting to see if the issues are severe due to a modelling course. 
        \interviewquote{when you're doing so assignments and everything with a group because everyone has a different point of view and there's going to be very messy}{GU\_S\_S2}
        %
        \interviewquote{Some people don’t like to draw., but we’re supposed to work together.}{BTH\_SAQ\_S1}
        %
        \interviewquote{but I think it would have been a lot better if we had all just sat down and done a class diagram and a sequence diagram, I think}{RU\_S\_S1}
        
        \item \textbf{Course issues:} Students mentioned their challenges with course structure:
        \shalini{We can check this with instructor's opinions about their course description}
        \interviewquote{assignment driven course}{RU\_G\_s1}
        %
        \interviewquote{we got to know all the basics and the whole idea and how it's supposed to look like, but not how to use it in the future on the bigger picture and the scale of the app}{RU\_G\_S4}
        %
        \interviewquote{For one course to have 500 book pages...you don’t have enough time to cover}{BTH\_SAQ\_S3}
        
        \item \textbf{Practice issues(by students):} Students mention that they don't have enough practice of modelling during the course. 
        \interviewquote{We did it in phases, so I didn't really get much of experience on that because I was just following the sketch that we got in the lectures and the classes and just tried to gather the basic stuff, designing in my head}{RU\_G\_S3}
        %
        \interviewquote{It was one semester, we got to know all the basics and the whole idea and how it's supposed to look like, but not how to use it in the future on the bigger picture and the scale of the app. That was the biggest challenge when they're using it}{RU\_G\_S4}
        %
        \interviewquote{What will be your previous state and what will be in your next step...that was really challenging...we have to submit three times}{BTH\_SAQ\_S2}
        \item \textbf{Guidance issues (course related):} students mention challenges due to lack of guidance. 
        \interviewquote{Felt like when it really came down to it, the UML part should have been a lot more. Because that we ended up using a lot}{RU\_G\_S1}
        %
        \interviewquote{just the syntax maybe, knowing what do you put in it and stuff}{RU\_S\_S2}
        %
        \interviewquote{Maybe because it's the first year, this is the first introduction to the subject, so people miss a lot of points, but if it had another level, teach people more, and take their hand more to do these diagrams themselves, that would be good}{RU\_G\_S3}
        %
        \interviewquote{I didn't get enough experience. We just had a big group project, which was three weeks to two weeks long. I think the teacher also didn't give much feedback on the assignments so I think that was missing, a feedback part from the teachers, if we were doing it correctly, if it doesn't look good, or anything like this. I think the experience is missing.}{RU\_G\_S4}
        \item \textbf{Issues regarding modelling purpose:}
        
        \item \textbf{"Don't know what to do": }
        \item \textbf{Others:}
        
        \subsubsection{Preference/Why}
For example, 
\interviewquote{I always have paper and pen, so even if I can't use the software, I can sketch stuff, it's casual sketching. It's nothing professional, but at least for me to communicate to think about the problem, and model it}{RU\_G\_S3}
%
\interviewquote{What we usually start doing is defining everything on a real high level. Start defining just the names of the classes or everything. That's basically getting the whole picture together and then we go into more detail}{RU\_S\_S1}
%
\interviewquote{Yeah, yeah we used that because it was um..prettier, than this is the whole perfectionism thing with um, it was prettier than coding}{RU\_G\_S2}
%
We found suggestions regarding the course as well:
\interviewquote{I think actually giving people the freedom to do what they want with the tools is really nice, because some people actually liked drawing it on an iPad or something}{RU\_S\_S1}
%
The category helps to understand the individuality which eventually brings the style from a modeller. 

%results


\begin{itemize}
	\item RQ1: What are the main difficulties or challenges a student faces while modelling?\newline
	%
%As mentioned above its hard to directly point out student challenges as we conducted 16 semi structured interviews and the data we collected are diverse. Semi-structured interviews are suitable for exploring a certain population's perception of a specific topic. In our case, we interviewed students from 3 different universities across 2 countries, and they were distributed among 5 courses. Hence, we had to adapt to the situation. While we used direct questions like, \emph{What challenges did you face during your modelling experience?} we also ask them conceptual questions like \emph{In what situation modelling won't be useful?}. We understood getting a direct answer would be impossible; therefore, we aimed for students' overall experience. 
	%
	
After analysing the data using in vivo coding, we observed 3 main groups of challenges:
\newline
	\textbf{Modelling is time consuming} \newline
	\interviewquote{modelling takes a lot of time from us}{GU\_S\_S2}
	\textbf{Unable to understand the purpose of modelling/ what diagram to use? confusion about syntax, technical constraints} \newline
	
	\textbf{Personal issues/ communication problems in group} \newline
	%
	Figure x shows students statements and their distribution among the three challenge groups. While challenges from the first group are most common among students, we did not find any solid reasons to argue those challenges. For other groups, we demonstrate the reasons behind those challenges in the next section.
	%
	\item RQ2: What are the potential reasons behind these challenges? \newline
	%
	
	\item RQ3: What is the student's perception of modelling? \newline
	%
	
	\item RQ4: What are the influencing factors behind a student's perception of modelling? 
\shalini{Points to consider}	 
	\item Background of a student and its influence on learning modelling:
	\item The results will be in three sections: In the first section, we will describe the categories from two data sets (students and instructors); in the second section, we will explain how these categories complement each other. For example, matching the student challenges from both data sets: checking if instructors acknowledge what's been troubling the students most. Note that we are not trying to come up with who's right, but just understanding the current situation. Another example is to check whether we can find potential reasons for the problems mentioned by students from instructors. The challenges instructors face, can they be considered as reasons for student challenges? or this is an addition to general challenges for modelling courses. Students mention group issues; are instructors aware of those? Is there any common topic between students' preferences and the instructor's suggestions? 
	%
	
	Finally, in the third section, we will discuss what we think are the student challenges and how we should proceed towards a solution? 
	\item Make a chart describing students to challenge from the above-mentioned categories regarding students' challenges. The chart will help us to understand the most common challenge among students. 
\end{itemize}



==> Extra stuff/OldLongerInterview.tex <==
\subsection{Interview Guide}
The interview is divided into three sessions. The first session starts with a small introduction presented by the interviewer which consists the following points:
\begin{itemize}
    \item First the interviewers introduce themselves.
    \item Then the interviewers express their purpose.
    \item Then they explain the whole procedure. 
\end{itemize}
After this we proceed with the interview. Our interview guide contain three sets of questions:
%GL: contains
Introductory questions (I), model questions (M) and task questions (T). 

\begin{itemize}
    \item I1: Which degree are you currently pursuing? (in which major?)
    \item I2: Which elective courses have you taken or are taking?
    \item I3: What is your experience in modelling?
    \item M1: What do you know about Model Based Engineering (MBE)?
    %GL: We should look at this before deciding on the interviewees. It depends a lot on the courses they've taken whether or not they can answer this.
    \item M2: How much modelling you have done in the past? Any project work? practical assignment?
    \item M3: What are the challenges you faced during that application? 
    \item M6: Do you think modelling was useful? Why?
    \item M7: Which modelling tool you prefer the most? Why?
    %GL: Relation to RQs?
    %SC : skipped.\item M8: If I tell you to rate your modelling course out of 5, 5 being the highest what will you give? 
    %GL: What do you want to get out of this question (and the one below)?
    %SC: skipped. \item M9: Why such rating?
    \item M8: If it's up to you, what will you change in the course?
    \item M9: 
\end{itemize}
% SC: I'll add the hypotheses-questionnaire link later.
After completing introductory and model questions, we take a short break (I hope with coffee and some snacks!). This break provide the interviewer some time to take a look at the answers and if needed make some changes. In the second session, we give students some design problem and ask them to solve it by modelling. We give them white papers and pencil, just to draw their ideas or approach for solving. This session is for 20 minuets and students are provided with internet. The interviewers will be in the same room the whole time for any questions or help. 

\subsubsection{Design Problem}
%GL: Any thoughts on how much time this might take? I believe you did a similar model for your MSc, right? How long did that take you?
%GL: What will the purpose of the model be? What should it be good for? Simulation? Code generation? Communication between people?
%GL: Instructions on notation, level of detail: Should they stick to a certain standard language? Should they care about syntax or not?

\chg{D}{The d}esign problem \del{again} is divided into three parts.
%
First\ins{,} \chg{we start with some requirements and students will model those}{the students will have to model a number of requirements}.
%
Then\ins{,} we will add \chg{new}{additional} requirements for the next two parts.
%GL: I only see one part here. What's the second one?
The students \chg{would}{will} be informed about this beforehand so they can \ins{model the problem likewise}{create the model to be easy to modify}.
%
This design problem is to see how model construction affect system changeability, maintainability and improvisation. 
%GL: What is?
%GL: Improvisation is not a system quality, so it doesn't quite fit here.

Students have to model a smart city cross junction traffic system, with autonomous vehicles and pedestrians.
%GL: Why autonomous vehicles? What does it add to the problem?
For simplicity we can assume that only autonomous private vehicles are travelling on the road, no public transportation.
%GL: How would it change the difficulty if you were to introduce public transport (it's still autonomous...)
The following requirements should be implemented:
\begin{enumerate}
    \item Cars/pedestrians can go to any of the three directions: straight, left and right.
    \item The cars should maintain a predefined distance between themselves.
    \item No accidents should happen with cars or pedestrians.
    \item Cars with emergency like ambulances are given priority to go forward.
    \item If a car breaks down in the middle of the road, that shouldn't cause any road blockage.
\end{enumerate}
%GL: So they should not really model the junction only, but also the car behaviour, right?
The first three requirements are given initially and then we will introduce the last two requirements in the next parts respectively.
%GL: Does this mean one requirement will be added, they get some time, and then the second one gets added? Also, I would expect this sentence in the previous paragraph (since there you talk about requirements being added).
Apart from the requirements the students can add additional functionality, but they must explain \chg{them}{the reasons for adding this functionality}.
%
The students are allowed to use internet, also the interviewers will be present all the time, so students can ask queries during the session. 

When the students are done with the second session, \chg{they'll}{they will} hand their respective papers to the interviewers. Then the third session will start with the following questions:
\begin{itemize}
    \item T1: What was your opinion regarding the problem?
    \item T2: Do you think you had enough information to solve the problem?
    \item T3: The approach you have used here, walk us through that.
    \item T4: Can you imagine any other styles that could be used to solve this problem?
    \item T5: If i asked you to add/modify three things from the given problem what will you choose? 
    \item T6: Why would you use that tool?
    %GL: Which tool? This question comes a bit as a surprise...
    \item T7: According to you what is good and bad with this tool?
    %GL: Why just one?
    %SC: changed it.
    %SC: skipped.\item T9: Tell me step by step how would you solve the given problem. 
    %SC: We can check side by side their paper to make sure what ever they wrote they understood it.
    %GL: Might be tricky. Maybe we can combine that with T3?
    \item T8: When we \chg{add}{added} the 2nd requirement\ins{,} what problems did you face? Similarly\ins{,} with the last added requirement\ins{,} what problems did you face?
    \item T9: If you go back, memorize the whole problem and your design, how you feel about it?
    %GL: Do you really mean memorise here?
    %SC: no, it's more like seeing the whole problem and solution at once, not literally "memorize".
    \item T10: Which part was the most difficult to model? Why?
    \item T11: Now that you have all the information about this problem, if I asked you to create different models to design this, how would you modify your answer?
\end{itemize}

\section{Theoretical Framework}
\subsection{Hypotheses}
The nature of our study is deductive \cite{bookRuneson2012} which means we start with some existing hypotheses created from related work and other research.
%GL: Redundant - you had something similar before.
There are some student studies in MBE that provide us information about either some specific challenge \cite{Pourali2018AnEm} or to develop a course for students \cite{Poruban2015Teaching}. Our study is not bound to any of such particular area, rather than it is an open platform for students to express their knowledge, problems and willingness towards MBE. To support this, we develop the following hypotheses:
\begin{itemize}
    \item H1: We propose that students are not receiving enough knowledge about model construction from a normal university level modelling course.
    % SC: Is it too harsh to say this statement?
    %GL: No, its fine - but you have to explain/argue this point. So after the list of items, I would explain each of them (and where it comes from). But I would rephrase "not receiving enough knowledge" to aim specifically at model construction, not modelling in general.
    \item H2: We propose that students are not willing to do modelling, because they lack the knowledge to do so. 
    \item H3: We propose three difficulties: tooling issues, lack of notation knowledge and lack of training. 
    \item H4: We propose that, given enough support, students will make use of MBE.
    %GL: Fair enough, but hard to answer in this study.
\end{itemize}
Research questions mentioned in section 1 are linked to the hypotheses. 

H1- RQ1

H2- RQ1, RQ2

H3- RQ2

H4- RQ3


==> Extra stuff/protocol.tex <==
\section{Protocol}
\begin{itemize}
    \item (25th May) SC took two pilot interviews with Majd and Elli. After discussion with GL, changes are made in the interview guide. Some of the main changes are insertion of the explanation of software modelling, removal of questions related to MBE. 
    \item (10th Aug) SC took another pilot interview with Zakarias. No changes required in the interview guide.
    Note: if students are not clear about the challenges/difficulties, ask additional questions to get more information.
    \item (19th Aug) SC took an interview of Marta, teacher of GHOH course. Marta suggested another teacher, Skuli Arnlaugsson (he is teaching the modelling part in GHOH course). 
    \item (20th Aug) SC started interviewing students. Interviewed one student from HUGB course. No changes required in the interview guide.
    \item (26th Aug) GL and SC listen to Zakarias's interview (12:58-22:25) and following issues are discussed:
    \begin{enumerate}
        \item Start transcribing the interviews.
        \item Coding (writing memos, try to find out as an interviewer what surprised you, disturbed you, figure out the "clear" statements e.g. "not taught right from day 1" In-vivo coding )
        \item Note for SC: Don't interrupt students, let them speak. When they ask you, "do you get it?" or "do you understand?", don't just say yes, try to repeat what they just said to get more information out of them. Do not rush! Don't suggest!
        \item Changes in InterviewGuide questions: If they say they don't understand the context of a diagram, add sub questions regarding the problem given to them. Otherwise no changes are made.
    \end{enumerate}
    \item (4th Sept) SC did an interview with Skuli, another teacher of GHOH course. 
    Findings:
    \begin{enumerate}
        \item He believes students get much knowledge from the course but as a "breadth wise" not "depth wise". 
        \item Might do another interview with him at the end of the course, to know his current experience.
        \item The modelling part was focused just on UML stuff. 
    \end{enumerate}
    \item (9th Sept) SC transcribed both student interviews and following points popped up!
    \begin{enumerate}
        \item Try to assemble the source of their challenges: 
        \item How requirements were given to them? Did that have any impact?
        \item Are they "encouraged" to utilize the diagrams properly? 
        \item Upon asking "was modelling helpful to you"? how are they responding?
        \item How modelling helped them? According to one student: " Because we had this physical model representation of the program." So they are thinking about the code-point of view, but is there any other angle to it? 
        \item Change in the InterviewGuide: Maybe we can go in little detail with questions, like "what was the given problem?" "How the requirements were given to you?" "How many people were there in your group?" And then maybe come down to challenges. 
    \end{enumerate}
    \item (23rd Sept) What do we know so far from both the student interviews:
    \begin{enumerate}
        \item For both of the students, it was their first modelling course. Student 1 was new to coding as well, but Student 2 is an experienced programmer. How does it affect their learning? It affected their sequence of learning, and both experienced the benefits of modelling differently.
        \item Student 1: Modelling helped student 1 to understand the problem and how to solve it. I think modelling somehow cleared her assumption about coding as well, "And like getting the connections right was very important to the coding." 
        %
        \item Student 2: "But if you making something that you create something, you read out of it and you, you look at it and stuff, then you gonna have to use programs to really just  trace back n forth through the, through the model to better understand what you doing." Modelling is useful for student 2 w.r.t coding. 
        \item What do students expect from a modelling assignment?
        \item Unfamiliarity with notations, 
        \item "Um, a lot of the drawings I make for me personally as I code, which are obviously… I mean they are smaller and more like, but they are personal to me so I understand everything I am doing, I understand my drawings but nobody else does"-Student 1 (line 94). Communication, a common way to create models (although it is a beginner's course and it would be unfair to expect that sort of communication from students).
        %
        \item "Because we had this physical model representation of the program." "...have this physical representation of the code" - student 2.
        Not the problem, but the program/code.
        \item "But like, like I said one third of it was UML. Felt like when it really came down to it, the UML part should have been a lot more. Because that we ended up using a lot." Modification?
        \item Aspect of analysis: \textbf{The beneficial side of modelling according to a student.} how many categories are there?
        \item For student 1: Changing the model helps because then you don't have to change the code.
        
        For Student 2: Changing the code was easy but it was an extra burden to go behind and change the uml.
        \end{enumerate}
        \item (Feb) We decided to start student interviews again. 2nd Feb GL posted on the discord channel for his web programming course's students. Till now (15th Feb), SC interviewed total 3 students who are from web programming course, two of them had taken Marta's course (GHOH) in the past, and one of them had taken SRAD course in past. 
        \item (Feb) We have contacted 3 instructors from different institutes for future interviews and made a requirement list for the case study (for recruiting students and also for compensation):
            \begin{enumerate}
                \item Omar Bahy Badreddin and Rahad Khandoker (for student interviews and also future collaboration, Texas, USA); Skúli Arnlaugsson (RU, teacher of SRAD course) and Birgit Penzenstadler (Germany).
                \item We are studying multiple cases (university courses that cover a substantial amount of modelling, on undergrad level), for each case, we aim to interview the instructor (if multiple, the one who is most involved in the modelling part) and up to 10 students. It’s fine to mix students from multiple years, unless there were substantial changes between the years. Covid is maybe an argument here, but I would actually say it should be fine nevertheless.
                \item Students sign an informed consent form and are guaranteed the option to withdraw at any time from the study. Participation is entirely voluntary. As a part of the consent, they have the option to approve/decline that we publish the full (anonymised) transcripts of the interviews. If needed, we have to get ethics approval from the respective university, according to state/country policy.
                \item As an instructor, you do not get to know who of the students is participating, to avoid any kind of potential bias in grading the students. You would advertise the study to your students and explain the conditions (or SC/GL would do that), but volunteers would then directly contact SC.
                \item The students receive compensation. We cover the compensation. We offer either cinema vouchers or donate the corresponding amount to charity.
            \end{enumerate}
        \item (15th Feb) We decided to present our case study to another course, we have already interviewed one student from that course. 
        \item In total we have interviewed 4 students from GHOH course (their instructors), one student from SRAD course (haven't interviewed the instructor). 
        \item (9th March) SC and GL started analysing the interview data (RU students, 5) and we found the following:
            \begin{enumerate}
                \item \textbf{Same Page:SP} Modelling helps everyone to be on the same page. Mostly according to students they used modelling to communicate between themselves.
                \item \textbf{Planning Ahead:PA} To understand the given problem, later they implemented the model (although that was required for the course).
                \item \textbf{Handling complexity:HC} Another approach from students. It's their way of understanding the problem or the complexity of the problem. One of the purpose of modelling for students. 
                \item \textbf{Usefulness:US} Not so much data here; although changing the model often seems a problem for students, they still think it's better to make changes at the modelling level than later at programming. 
                \item \textbf{Don't know what to do:DKD} This group of statements explains that students are actually confused about modelling. One of the main challenges students face is to change the model multiple times. They even changed their diagrams after programming. "...lot of people thought it was (class diagram) kind of pointless to begin with...in the very end they pretty much didn't follow the class diagram at all."
                \item \textbf{Timing:T} Modelling is time consuming. 
                \item \textbf{Challenges in general:C} "We are just drawing diagrams"-clueless about the purpose. They are questioning what is the need to learn different types of diagrams? 
                \item \textbf{Practice/Guidance:P/G} They learn about modelling but don't get to experience modelling: lack of practical exposure, different outcomes from different teacher, short practise time.
                \item \textbf{Group Issues:GI} The assignments were in group, different students have different opinions. Less professionalism. 
                \item \textbf{Course issues:CI} Due to course structure, less time to learn.
                \item \textbf{Model Purpose:MP} "Design first, the implement", "school forces us to model..." The purpose of modelling to students. 
                \item \textbf{Preferences:P} How the students perceive modelling and how they complete the assignments through modelling (very close to style) "...we sometimes just get something based on UML but it is not completely UML"
                \item \textbf{Solve by Modelling: SM} It is one of the approaches taken by students, trying to solve the given problem by modelling. It is related to MP, as students learn to design first.  Do they understand the problem through modelling first? or just start with modelling cause it was the requirement for a course?
            \end{enumerate}
            \item Do the students understand a problem by modelling or start with modelling cause the course demands "design first, then implement". If we see PA (planning ahead), it seems students use modelling to understand the problem, but they complain the course demands design first. 
            \item (15th March) SC interviewed another student from Skuli's course. He was very new to modelling, not much to share. 
            \item (15th March) SC interviewed Skuli for the 2nd time. 
            \item (16th March) SC interviewed 3rd student from SRAD.
            \item (1st April) SC interviewed a student from Birgit's course at Gothenberg. The student took that course and also later appointed as TA under Birgit for the same course.
            \item (15th April) SC interviewed 5th student from Marta's course.
            \item (20th April) SC interviewed Birgit (I4) and presented her study in Birgit's class (SAD).
            \item (30th april) SC interviewed 2nd student from SAD.
            \item (15th Sept.) SC analysed rest of the students from GHOH (RU\_G\_S5) and SRAD (RU\_S\_S2, RU\_S\_S3) and update the coding. 
            \item (27-30th Sept) SC mailed Daniel from BTH for probable student participants. We got three instructors and their respective courses. 
            \item (30th sept) SC and GL did coding for instructors. SC started analysing her invivo coding, 5th Oct SC and GL will sit together and discuss about it. 
            \item (12th Oct) SC presented her study in Nasir's course (PA2550) at BTH. We didn't mention anything about compensation. 
            \item (15th Oct) SC got two volunteers from PA2550. 
            \item (18th Oct) Interviewed first student from Nasir's course.
            \item (19th Oct) Interviewed second student from Nasir's course.
            \item (8th nov) Interviewed Nasir. Got two new students from his course.
            \item (9th Nov) SC interviewed 3rd student from Nasir's course.
            \item (10th nov) Grouping the students (experienced, new to course, wise?), have a high level abstract that connects the result. Check with the categories, maybe they have different values for different students.
            \item (12th Nov) SC interviewed Usman (I6), instructor of SAQ.
            \item (15th Nov) SC interviewed first 2 students from SAQ. First interview was very interesting.
            \item (29th Nov) SC interviewed 3rd student from SAQ. 
            \item (24th March) Sorting out categories for student challenges. Right now we have few categories those are fixed and some that needs some merging and notification. Fix categories are: modelling is time consuming, rework of wrong models, tooling, lack of cooperation,Lack of interactivity, Common point of view/interpretation, tight schedule and not useful. 
            \item Categories that we do need to work on: Don't know how to model/what to do, suitability of modelling, complexity of notation/UML, guidance, model purpose. 
            \item three non important categories: remote issues, rest and Inappropriate examples/context. 
        
\end{itemize}

==> Interview guide/Interviewguideinstructor.tex <==
\subsubsection{Interview with instructors: A view of the course}
\todo[inline]{Introduce Marta and the course (Software Analysis and Design). Also why it is important to take an interview of her for the course/my research}
%
\begin{enumerate}
    \item Could you shortly describe which topics you cover in your course?
    \item Regarding modelling, what are you covering in the course?
        \begin{enumerate}
            \item Are you teaching modelling notation (e.g., UML diagrams)?
            \item Are you teaching how to draw those models (example: identify nouns/verbs in a text to draw class diagrams)?
            \item Are you teaching how the models relate to code?
            \item Are you teaching semantics of modelling notations?
        \end{enumerate}
    \item Roughly how much time is spent on modelling in your course?
    \item Regarding modelling, what is covered in assignments or exam?
    \item How do you think students perceive the modelling part of the course?
    \item What do you think are the things that students struggle with (with respect to modelling)?
    \item What challenges are you facing when teaching modelling?
    \item How do you think this could be improved?
\end{enumerate}

\subsubsection{Follow-up Interview}
\begin{enumerate}
    \item What is your overall experience from the previous course?
    \item Are you involved with the theoretical part of the course? Or the practical part or both?
    \item From your experience which part of the theory lessons you find most challenging? Why do you find it challenging?
    \item What are the most common questions about modelling you get from the students?
    \item How do students perform in the practical sessions?
    \item What are the assignments they followed in the course? What is the outline of the assignments? (like rules, how it was conducted)
    \item What kind of complaints you got from students during the course? During the practical sessions? (I think TA's can answer this question better)
    \item Did you observe any common challenges among students regarding the assignments? What are those challenges?
    \item What is your impression of their final submission?
    \item Do you want to change anything from the course? If yes, then what is it and why?
\end{enumerate}

==> Interview guide/Interviewguidestudent.tex <==
The purpose of this interview is to gain knowledge regarding the research questions. Duration of the interview is 40 minutes.
\subsubsection{Student Interview Guide}
The interview starts with a small introduction presented by the interviewer(s) which consists the following points:
\begin{itemize}
    \item Ask whether it is OK to record the interview.
    \item First the interviewers introduce themselves.(2 minutes)
    %GL: "I try to find out how to create models in the best possible way" - maybe "I try to understand better how models are being created."
    \item Then the interviewers explain the study's purpose, the ongoing research and the research questions. (5 minutes)
    (The purpose of the research is to understand how models are created. The research is broken down to three groups. First we figure out how models are created? Second, we will investigate the challenges behind model creation. This interview is part of that second group. Finally, with the information we will collect from previous two studies, we will make a guideline for model creation. The purpose of this study is to gather information about model creation from students. Information like different challenges/ difficulties a student faces while modelling, according to a student what are the reasons behind those difficulties, students perspective on the challenges of model creation...)
    \item Then they explain the whole procedure of the interview. (3 minutes)
\end{itemize}
This part takes 10 minutes. After this we proceed with the interview in the following manner:
\subsubsection{Part I: Introductory Questions}
The duration of this part is 10 minutes.
\begin{enumerate}
    \item I1: Which degree are you currently pursuing? (in which major?)
    %GL: How useful is this question? What do we get out of it?
    %SC: deleted. (no questions for elective courses)
    \item I2: Have you worked in industry? If yes, what role/domain?
    \item I3: Do you have any experience with modelling? What kind of experience do you have with modelling?
    %GL: Elli's answer was somewhat expected: "What do you mean by model?"
    %SC: After proper explanation of the research they should not have this question.
    %\todo[inline]{Depends. I don't see in the explanation that you explain what you mean by modelling. So they could still ask that...}
    %GL: We need to have a good answer to that. "Represent the phases as a model" is a bit fuzzy. "What I had in mind were database models" - well that is also a model.
    %SC: ask about diagrams. go in details.
    %GL: Not a question, but at this point in the interview, you need to remember that there is syntax, semantics, and pragmatics of modelling languages - you might have to dig a bit deeper to find out what they covered/know.
    \item I4: Go in detail with the experience, ask about syntax, diagrams that they had used before.
    
\end{enumerate}
\subsubsection{Part II: Model Questions}
Duration of this part is 20 minutes. Before going into the modelling questions explain what software modelling is. (In which modelling we are actually interested in?)
What is your idea of software modelling?
Models are abstractions used to represent the development, the design of the software. It helps developers deal with the complexity of the problem being investigated or the solution being developed. "Modelling is like building a house. You start by drawing a rough sketch of the floor plan and layout of the rooms and floors. The drawing is your modeling language and the resulting blueprint will be a model of your final design. You will continue to modify your drawings until you arrive at a design that meets all your requirements. Only then should you start cutting boards or writing code. " "UML is a modelling language, not a development process – it gives you a set of techniques, but does not prescribe whether or how these techniques should be used during development."
We are interested in high level modelling, graphical modelling.
%\todo[inline]{Suggest: Remove MBE stuff, more depth on software modelling}
\begin{enumerate}
    %M1: Do you know the term Model Based Engineering (MBE)?
    %GL: Is it important? You don't really come back to it later again.
    %SC: Should we completely remove MBE?
    %\todo[inline]{Up to you. The question is: Why is it here? Are you planning to answer anything with this question? If not, maybe remove.}
   %M2: (If M1=Yes)What do you know about MBE?
    %If M1=No; explain MBE.
    \item M1: What experience do you have in software modelling?
    %GL: I do think we need to explain this before.
    %GL: We look at graphical modelling only.
    %\item M6: The project work you mentioned before regarding modelling, can you tell me that in detail?
    %GL: Why here? Why not directly when you ask about that?
    %SC: In that section I don't want to go in details with the answers. The introductory part of interview is just to know if they had any experience (what was it?). Also if they mention more than one 1 project work, it would be better to hear them in details. 
    
    %GL: Question about the approach: Is not necessarily useful. The answers are either made up, or too abstract.
    
    \item M2: What did you like from your experience?
    %\todo[inline]{Connection. The previous question is "What do you think software modelling is?". So if you ask this question precisely as it's stated here, no one will understand what "that project" is.}
    %GL: Enjoy is strange wording. It's more about what it was useful, what you liked, etc.
    \item M3: What challenges did you face during your experience?
    %GL: Majd answered not what the challenge is, but what the solution is ("you need a goal")
    \todo[inline]{Be careful here, if they answer like majd, make sure to get back on challenges.
    
    Make them talk about at least one of their experiences with software modelling, if they don't go straight to challenges, at least we know the stories and can dig out the dirt!}
    
    \item M4: In your opinion what are the reasons behind these challenges?
    \item (If needed): When you are using a modelling notation what typically troubles you? (notations like UML)
    %GL: Elli answered with something that was not related to modelling. So then this question does not really make sense --> You have to adapt the questioning.
    \item M5: How was your experience with modelling tools? Tell me about the tools you have used in the past.
    \item M6: What did you like and dislike about each of those tools?
    %GL: Careful with leading questions "The tool is free..." "And you understand how the tool works? It's easy..." "It's easy"
    \item M7: For which purposes/in which situations (in SE) do you think modelling is useful? When is this not the case?
    \item M7.1: How did you use modelling in your course?
    \item M8: In your case can you tell me of an experience where you found modelling useful?
    %\todo[inline]{"Any similar" - similar to what?}
    %\item (If needed): What is your approach when creating a model?
    %\todo[inline]{You'll have to explain that question, I think.}
    
    %SC: We can use these questions if we don't get enough answers from previous ones.
    %SC: Bit tricky, might need to explain.
    \item M9: What advantages and disadvantages do you see in modelling?
    %GL: Majd went into code generation, a very specific way of modelling.
    \item M10: Did you get enough knowledge about modelling from the courses you have taken on the topic?
    %GL: Majd: "I'd like to apply all diagrams"
    \item M11: What was missing from those courses?
    %GL: Needs to be concrete. We need to have context on the courses.
    \item M12: How would the perfect modelling course look like?
    \item M13: Do you have any comments or suggestions?
    %GL: Last question in Elli's interview is leading "Don't you think that..."
    %GL: "Do you think all the modelling tools are nice?" - asks for a negative answer. What do you really want to ask?
\end{enumerate}
%\subsection{Part III: Survey}
%GL: Skip the survey. If you have any quantitative questions, just ask them. But I'm not sure this makes sense - you typically don't have many people to interview, so the numbers won't be meaningful.
%SC:Skipped!!At the end of the interview students are given a survey form to express their experience about the interview. Students get 5 minutes to fill out that form. This is the last activity of this whole interview, after this the interviewer thanks the students for participation and end the interview. The structure of the survey form is given below:


==> taskslefttodo.tex <==
\begin{enumerate}
    \item Introduction: Revision needed (there are surveys but no case studies, depth is missing)
    \item Related Work: Need more info (e.g. problem domain)
    \item Method: Needs reductions. 
    \item Results: work in progress...
    \item Conclusion: need to write. 
    \item Haven't received the assignment details from Skulli, Nasir and Usman. second reminder sent.
    \item If not ESEM, MODELS abstract deadline is 11th May, full paper 18th May. 
\end{enumerate}

\section{Questions?}
\begin{itemize}
    \item RQs: I prefer just two questions: perception and challenges. We can discuss reasons or solutions of challenges, but not as a separate RQ.
    \item If we get the assignments, how to proceed with them?
    \item Option to review the results to the interviewees.
        Check if anything else left to do. 
        Publication of the transcripts: change them, hide personal details
        if model people are stupid, send it to journal. 
        compare the pictures
        Education come first
        Is industry influencing the learning practice, as no one use it in industry. 
        they are not discussing the diagrams, everyone in a group makes different things. Not seeing the purpose of it. 
        How does the data here compare with industry? 
        
        \item What is in the assignments?
        Tooling? Time schedule-modelling takes time?
        Assignments layout- how many times they have to submit?
        Domain? are students mature enough for it?
        Practice- does the assignment allow practice?
        Assignment purpose: 
\end{itemize}
